On the convergence of Block Majorization-Minimization algorithms on the Grassmann Manifold

The Majorization-Minimization (MM) framework is widely used to derive efficient algorithms for specific problems that require the optimization of a cost function (which can be convex or not). It is based on a sequential optimization of a surrogate function over closed convex sets. A natural extension of this framework incorporates ideas of Block Coordinate Descent (BCD) algorithms into the MM framework, also known as block MM. The rationale behind the block extension is to partition the optimization variables into several independent blocks, to obtain a surrogate for each block, and to optimize the surrogate of each block cyclically. The advantage of the block MM is that the construction and successive optimization of the surrogate functions is potentially easier than with the non-block alternative. The purpose of this letter is to exploit the geometrical properties of the Grassmann manifold (a non-convex set) for the purpose of extending classical convergence proofs of the block MM when at least one of the blocks is constrained in this manifold.

==> Sections/unused.tex <==
It is highlighted that the key steps in our proof, and the main difference with the non-Riemannian optimization proof, are the derivations up to equation (\ref{eqn:conv_cond}). The properties of geodesics in the Grassmann manifold (with the unique minimizer assumption on the majorants) are sufficient conditions to ensure the convergence of the block MM. Other manifolds that share these properties also admit a similar convergence proof.




It is shown in this paper that the block MM framework also converges for variables constrained in the Grassmannian. Some of the classical assumptions about the majorant functions that are needed for the convergence of block MM algorithms are generalized within the geodesically convex optimization paradigm. This letter gives some additional insights to include the MM framework into this paradigm as we conjecture that this convergence proof can be extended to other Riemannian manifolds that have similar properties to the Grassmann manifold.




The previous definition implies that the sublevel set given by:
\begin{equation}
    S = \{\mathbf{X} \in \mathcal{G}: f(\mathbf{X}) \leq \alpha \},
\end{equation}
is geodesically convex. 










Let a function $f_{eg}(\mathbf{U}, \boldsymbol{\mu})$, where $\mathbf{U} \in \text{Gr}(N, D)$ and $\boldsymbol{\mu} \in \mathbb{R}^{N}$, be such that its sublevel set is compact and that is majorized by:
    \begin{equation}
        \label{eqn:majorant_example}
        g_{eg}(\mathbf{U}, \boldsymbol{\mu} | \mathbf{U}_i, \boldsymbol{\mu}_i) = \text{tr}\left(\mathbf{U}^T \mathbf{G}(\boldsymbol{\mu} | \mathbf{U}_i, \boldsymbol{\mu}_i ) \mathbf{U} \right),
    \end{equation}
    where $\mathbf{G}(\boldsymbol{\mu} | \mathbf{U}_i, \boldsymbol{\mu}_i )$ is a matrix that is constructed using the $i$-th iterates and $\boldsymbol{\mu}$. Then, alternating between the optimization of $\mathbf{U}$ and $\boldsymbol{\mu}$ in (\ref{eqn:majorant_example}) results in an equivalent algorithm as the one depicted by (\ref{eqn:MM_update_general}). Hence, Theorem \ref{theo:convergence} ensures its convergence to a locally optimal point of $f_{eg}(\mathbf{U}, \boldsymbol{\mu})$. The setting in this example is depicted in known Signal Processing approaches, such as the one depicted by the Logistic PCA framework \cite[Section 5]{dimensionality_reduction_binary_data_natural_parameters} or in a generalized robust subspace recovery (similar to the one depicted in \cite[Section V-C]{mm_stiefel}), where a majorant similar to (\ref{eqn:majorant_example}) is obtained after rearranging terms from an upperbound of $f_{eg}(\mathbf{U}, \boldsymbol{\mu})$. See \cite{Truncated_power_method_sparse_eigenvalue, Nonconvex_approach_exact_efficient_multichannel, Dual_principal_component_pursuit} for alternative examples where Theorem \ref{theo:convergence} is proven useful to deal with non-convex constraint sets.



    The canonical metric is relevant since the concepts of geodesics, distances and Riemannian connections emanate from it.





\subsubsection{Grassmann canonical metric}

Given $\mathbf{A}, \mathbf{B} \in \mathcal{T}_{\mathbf{X}} \text{Gr}(N, D)$, the canonical Riemannian metric on the Grassmann manifold is defined as:
\begin{equation}
    \label{eqn:metric}
    \langle \mathbf{A}, \mathbf{B} \rangle_{\mathbf{X}} = \text{tr}(\mathbf{A}^T\mathbf{B}).
\end{equation}


, and $\mathbf{H} \in \mathcal{T}_\mathbf{X} \text{Gr}(N, D), \mathbf{T} \in \mathcal{T}_\mathbf{Y} \text{Gr}(N, D)$ are the tangent vectors that point to $\mathbf{Y}$ and $\mathbf{X}$, respectively.






In recent days, there has been an increasing availability of information sources and computing power that is matched with emerging algorithms in the era of big data. Those algorithms are often built on the optimization of some cost function. In this context, frameworks are designed to face the following challenges \cite{big_data_review}: they must handle multimodal datasets, provide integrity to the final solution, be computationally fast, and scale efficiently. 
